adcc: A versatile toolkit for rapid development of algebraic-diagrammatic construction methods

ADC-connect (adcc) is a hybrid python/C++ module for performing excited state calculations based on the algebraic-diagrammatic construction scheme for the polarisation propagator (ADC). Key design goal is to restrict adcc to this single purpose and facilitate connection to external packages, e.g., for obtaining the Hartree-Fock references, plotting spectra, or modelling solvents. Interfaces to four self-consistent field codes have already been implemented, namely pyscf, psi4, molsturm, and veloxchem. The computational workflow, including the numerical solvers, are implemented in python, whereas the working equations and other expensive expressions are done in C++. This equips adcc with adequate speed, making it a flexible toolkit for both rapid development of ADC-based computational spectroscopy methods as well as unusual computational workflows. This is demonstrated by three examples. Presently, ADC methods up to third order in perturbation theory are available in adcc, including the respective core-valence separation and spin-flip variants. Both restricted or unrestricted Hartree-Fock references can be employed.

==> common.tex <==

% Packages
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{relsize}
\usepackage{tikz}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage[tight]{units}
\usepackage{textgreek}
%\usepackage{todonotes}
%\newcommand{\todoil}{\todo[inline,caption={}]}
%\newcommand{\MS}{\todo[size=\footnotesize,author=MS,inline,backgroundcolor=green!80,caption={}]}
%\newcommand{\MFH}{\todo[size=\footnotesize,author=MFH,inline,backgroundcolor=blue!40,caption={}]}
%\newcommand{\TF}{\todo[size=\footnotesize,author=TF,inline,backgroundcolor=pink!40,caption={}]}

%% Programming languages
\newcommand{\python}  {\texttt{python}\xspace}
\newcommand{\cpp}     {\texttt{C++}\xspace}
\newcommand{\ccc}     {\texttt{C}\xspace}
\newcommand{\fortran} {\texttt{FORTRAN}\xspace}
\newcommand{\julia}   {\texttt{julia}\xspace}

% packages
\newcommand{\adcc}      {\texttt{adcc}\xspace}
\newcommand{\adcman}    {\texttt{adcman}\xspace}
\newcommand{\pyscf}     {\texttt{pyscf}\xspace}
\newcommand{\psifour}   {\texttt{psi4}\xspace}
\newcommand{\psifournp}   {\texttt{psi4numpy}\xspace}
\newcommand{\numpy}     {\texttt{numpy}\xspace}
\newcommand{\scipy}     {\texttt{scipy}\xspace}
\newcommand{\matplotlib}{\texttt{matplotlib}\xspace}
\newcommand{\pandas}    {\texttt{pandas}\xspace}
\newcommand{\molsturm}  {\texttt{molsturm}\xspace}
\newcommand{\libten}    {\texttt{libtensor}\xspace}
\newcommand{\libadc}    {\texttt{libadc}\xspace}

% Abbreviations
\newcommand{\ie}{\mbox{i.e.}\xspace}
\newcommand{\eg}{\mbox{e.g.}\xspace}

%% Quantum chemistry jargon
\newcommand{\SCF}{SCF\xspace}
\newcommand{\HF}{HF\xspace}
\newcommand{\ADC}{ADC\xspace}
\newcommand{\CS}{CS\xspace}
\newcommand{\cGTO}{cGTO\xspace}

% maths
\newcommand{\mat}{\mathbf}
\renewcommand{\vec}{\mathbf}

% Standalone bra and kets:
\newcommand*{\bra}[1]{\left\langle#1\right|}
\newcommand*{\ket}[1]{\left|#1\right\rangle}
%
% Bra and kets with something in the middle. 
% They do have to come as a pair!
\newcommand*{\mbra}[1]{\left\langle#1\middle|}
\newcommand*{\mket}[1]{\middle|#1\right\rangle}
%
% Ketbra and braket together:
\newcommand*{\braket}[2]{\left\langle#1\middle|#2\right\rangle}
\newcommand*{\ketbra}[2]{\left| #1 \middle\rangle \middle\langle #2 \right|}
%
% Creation and anihilation operators:
\newcommand*{\cop}[1]{\ensuremath{\op{c}_{#1}^{\dagger}}}
\newcommand*{\aop}[1]{\ensuremath{\op{c}_{#1}}}

\newcommand*{\Op}[1]{\ensuremath{\hat{\mathcal{#1}}}}
\newcommand*{\op}[1]{\ensuremath{\hat{\mathrm{#1}}}}

% Take the trace
\DeclareMathOperator{\tr}{tr}


==> minted.tex <==
\usepackage{minted}
\usemintedstyle{pastie}
\setminted{fontsize=\small,baselinestretch=1,frame=lines,linenos,breaklines}

